Test-Time Training Provably Improves Transformers as In-context Learners

Test-time training (TTT) methods explicitly update the weights of a model to adapt to the specific test instance, and they have found success in a variety of settings, including most recently language modeling and reasoning. To demystify this success, we investigate a gradient-based TTT algorithm for in-context learning, where we train a transformer model on the in-context demonstrations provided in the test prompt. Specifically, we provide a comprehensive theoretical characterization of linear transformers when the update rule is a single gradient step. Our theory (i) delineates the role of alignment between pretraining distribution and target task, (ii) demystifies how TTT can alleviate distribution shift, and (iii) quantifies the sample complexity of TTT including how it can significantly reduce the eventual sample size required for in-context learning. As our empirical contribution, we study the benefits of TTT for TabPFN, a tabular foundation model. In line with our theory, we demonstrate that TTT significantly reduces the required sample size for tabular classification (3 to 5 times fewer) unlocking substantial inference efficiency with a negligible training cost.

==> sections/problem_setup.tex <==
\section{Problem Setup}\label{sect problem setup}

\textbf{Notation.} Let $[n]$ denote the set $\{1,\cdots, n\}$ for an integer $n \geq 1$. We denote vectors and matrices using bold lower-case and upper-case letters, respectively, such as $\x$ for vectors and $\X$ for matrices. The element \(x_i\) refers to the \(i\)-th entry of the vector \(\x\). We represent the zero vector of size $n$ by $0_n$ and the zero matrix of size $m \times n$ by  $0_{m \times n}$. The operator $\tr{\X}$ represents the trace of $\X$.

\textbf{In-context learning and test-time-training.}
We consider the in-context learning setting with the input prompt
\[ 
\Z=[\Zprompt^\top ~\z]^\top\in\R^{(n+1)\times (d+1)},
\] 
where $\Zprompt=[\z_1 \cdots \z_n]^\top \in \R^{n \times (d+1)}$ is the context tokens, $\z_i=\begin{bmatrix}\x_i\\y_i\end{bmatrix}$ for $i \in [n]$, and $\z=\begin{bmatrix}\x\\0\end{bmatrix} \in \R^{(d+1)}$ is the query token. Let $\Xprompt = \begin{bmatrix}
\x_1 ~ \x_2 ~ \dots ~ \x_n
\end{bmatrix}^\top \in \R^{n \times d}$ be the data matrix and the corresponding labels are $\Yprompt = \begin{bmatrix}
y_1 ~ y_2 ~ \dots ~ y_n
\end{bmatrix}^\top \in \R^{n \times 1}$. Similar to previous works \cite{zhang2023trainedtransformerslearnlinear}, \cite{mahankali2023stepgradientdescentprovably}, \cite{ahn2023transformerslearnimplementpreconditioned}, \cite{li2024finegrainedanalysisincontextlinear},  we study the linear attention model as the sequence model:
\[
\SMi{\Z}{\W}
 = \left[ \Z \W_Q \W_K^\top \Z^\top \Z \W_V \right]_{n + 1} = \x^\top \W \Xprompt^\top \Yprompt   
\]
where the weight matrices $\W_Q \W_K^\top, \W_V \in \R^{(d+1) \times (d+1)}$ are defined as
\begin{align*}
\W_Q \W_K^\top & = \begin{bmatrix}
\W & \boldsymbol{0}_{d \times 1} \\ \boldsymbol{0}_{1 \times d} & 0
\end{bmatrix} & \W_V = \begin{bmatrix}
\boldsymbol{0}_{d \times d} & \boldsymbol{0}_{d \times 1} \\ \boldsymbol{0}_{1 \times d} & 1
\end{bmatrix} .
\end{align*}
We assume that the $\SM$ is \textbf{pre-trained} with the population data of $(\Zcont,\x, y)$ where $y$ is the label of the query token $\x$. Specifically, the row elements $(\x_i, y_i)_{i=1}^n$ and the $(\x,y)$ pairs are i.i.d. sampled from the pre-train distribution $\Dczpt(\bSibt)$. The distribution $\Dczpt(\bSibt)$ is characterized by the setting $y = \x^\top \betapt + \xi$ where the task parameter $\betapt$ is sampled from $\Nn(\boldsymbol{0}, \bSibt)$, the feature $\x$ sampled from the feature distribution $\Nn(\boldsymbol{0}, \bSix)$, and the noise term $\xi$ is sampled from $\Nn(0, \sigma^2)$. Specifically, the pre-training objective of the $\SM$ is
\begin{align}
    \Wst = \arg \min_{\W} \E_{(\x, y), (\x_i, y_i)_{i=1}^n \sim \Dczpt(\bSibt)} \left[(y - \SMi{\Z}{\W})^2\right] \label{eq:pop-loss-pre-train}
\end{align}
During inference, we test the $\SM$ with a new task parameter $\betatt$. Suppose that we observe a few samples of $\Sctt := \{(\x_i, y_i)\}_{i=1}^{(n+k)}$ pairs that are i.i.d. sampled from a \textbf{test-time} distribution $\Dcztt(\betatt)$ based on the task parameter $\betatt$. Formally, the pairs $(\x_i, y_i)$ are sampled by following the setting $y_i = \x_i^\top \betatt + \xi_i$ where $\x_i \distas \Nn(\boldsymbol{0}, \bSix)$ and $\xi_i \distas \Nn(0, \sigma^2)$. Before making the inference, we \textbf{test-time train} the model for the new task $\betatt$. For this, we apply a single-step gradient descent to the pre-trained matrix $\Wst$ on the data $\Sctt$ to obtain a test-time trained $\Wnew$. We measure the performance of the $\SM$ after and before the update with the following population loss on the new task parameter:
\begin{align}
    \Lc(\W) = \E_{(\x,y), (\x_i, y_i) \sim \Dcztt(\betatt)}\left[(y - \SM(\Z, \W))^2\right] \label{eq:pop-loss-new-task}
\end{align}
Our aim is to analyze the loss improvement from $\Lc(\Wst)$ to $\Lc(\Wnew)$ throughout the paper.

While applying a single-step gradient descent, we use the data $\Sctt$ by dividing it into two parts: We designate the first $n$ samples as the context, while we use the latter $k$ samples to form a query training set. Recall the definitions of $\Xprompt$ and $\Yprompt$, 
and we define the query training matrices as
\begin{align*}
\Xtrain = \begin{bmatrix} \x_{n + 1} \ \hdots \ \x_{n + k}  \end{bmatrix}^\top \quad \Ytrain = \begin{bmatrix}
y_{n+1} ~ \dots ~ y_{n+k}
\end{bmatrix}^\top
\end{align*}
with dimensions $\Xtrain \in \R^{k \times d}$ and $\Ytrain \in \R^{k}$. Similar to $\Zprompt$, we define $\Ztrain = [\Xtrain; \Ytrain]^\top \in \R^{k \times (d+1)}$. During test-time training, we take the gradient descent on the loss over the query tokens in $\Ztrain$ while using $\Zprompt$ as the fixed context across all query tokens. 
\begin{align}
\quad \mathcal{\hat{L}}(\Wst) = \sum_{i = n+1}^{n+k} (y_i - \SMi{\Z_{i}}{\Wst})^2 \label{eq:train-loss}
\end{align}
where $\Z_{i} = \begin{bmatrix}\Zprompt\\ \z_{i}^\top \end{bmatrix} \in \R^{(n+1) \times (d+1)}$ and $z_i = \begin{bmatrix}\x_i \\ y_i \end{bmatrix} \in \R^{(d+1)}$. The single-step gradient update on the loss function is provided in the following proposition:

%Our objective is to update the pre-trained $\SM$ with weight-matrix $\Wst$ by applying one gradient step on the loss calculated over the label mismatch over the $\Z_{\text{train}}$ by treating each of its elements as a query and using $\Z_{\text{prompt}}$ as the context. 



\begin{restatable}[Test-Time Gradient Step]{proposition}{onestepgradientupdate}\label{prop:one-step-update}
Consider the linear attention model with parameters $\W\in\R^{d\times d}$. Suppose the test-time training loss function is defined as in \eqref{eq:train-loss} where the prompt set is $\Z_{\text{prompt}}$ and the train set is $\Z_{\text{train}}$. Also define $\uprompt := \Xprompt^\top \Yprompt$. Then, for any step size $\eta>0$, the new parameter $\Wnew$ after one gradient-descent step from $\W$ is given by the rank-$1$ update
\begin{align*}
\Wnew = \W + 2\,\eta\, \Xtrain^\top \left( \Ytrain - \Xtrain\,\W \,\uprompt \right)
\;\uprompt^\top.
\end{align*}
\end{restatable}
As mentioned above, our aim is to analyze the loss improvement $\Lc(\Wnew) - \Lc(\Wst)$ with respect to the embedding dimension $d$, the sample size $n$, and the alignment between the distributions $\Dczpt(\bSibt)$ and $\Dcztt(\betatt)$.
